Pedestrian Detection: Domain Generalization, CNNs, Transformers and Beyond

Pedestrian detection is the cornerstone of many vision based applications, starting from object tracking to video surveillance and more recently, autonomous driving. With the rapid development of deep learning in object detection, pedestrian detection has achieved very good performance in traditional single-dataset training and evaluation setting. However, in this study on generalizable pedestrian detectors, we show that, current pedestrian detectors poorly handle even small domain shifts in cross-dataset evaluation. We attribute the limited generalization to two main factors, the method and the current sources of data. Regarding the method, we illustrate that biasness present in the design choices (e.g anchor settings) of current pedestrian detectors are the main contributing factor to the limited generalization. Most modern pedestrian detectors are tailored towards target dataset, where they do achieve high performance in traditional single training and testing pipeline, but suffer a degrade in performance when evaluated through cross-dataset evaluation. Consequently, a general object detector performs better in cross-dataset evaluation compared with state of the art pedestrian detectors, due to its generic design. As for the data, we show that the autonomous driving benchmarks are monotonous in nature, that is, they are not diverse in scenarios and dense in pedestrians. Therefore, benchmarks curated by crawling the web (which contain diverse and dense scenarios), are an efficient source of pre-training for providing a more robust representation. Accordingly, we propose a progressive fine-tuning strategy which improves generalization. Code and models can accessed at https://github.com/hasanirtiza/Pedestron.

==> sections/abstract.tex <==
\begin{abstract}
Pedestrian detection is used in many vision based applications ranging from video surveillance to autonomous driving. 
Despite achieving high performance, it is still largely unknown how well existing detectors generalize to unseen data.
To this end, we conduct a comprehensive study in this paper, using a general principle of direct cross-dataset evaluation.
Through this study, we find that existing state-of-the-art pedestrian detectors generalize poorly from one dataset to another.
We demonstrate that there are two reasons for this trend.
Firstly, they over-fit on popular datasets in a traditional single-dataset training and test pipeline.
Secondly, the training source is generally not dense in pedestrians and diverse in scenarios.
Accordingly, through experiments we find that a general purpose object detector works better in direct cross-dataset evaluation compared with state-of-the-art pedestrian detectors and we illustrate that diverse and dense datasets, collected by crawling the web, serve to be an efficient source of pre-training for pedestrian detection.
Furthermore, we find that a progressive training pipeline works good for autonomous driving oriented detector.
We improve upon previous state-of-the-art on \textit{reasonable}/\textit{heavy} subsets of \emph{CityPersons} dataset by 1.3$\%$/1.7$\%$ and on \emph{Caltech} by 1.8$\%$/14.9$\%$ in terms of log average miss rate (\LMR{}) points without any fine-tuning on the test set. Detector trained through proposed pipeline achieves top rank at the leaderborads of \cityperson{} and \ecp{}. Code and models can be accessed at \url{https://github.com/hasanirtiza/Pedestron}.




\end{abstract}

==> sections/abstract2.tex <==
\begin{abstract}
Pedestrian detection is used in many vision based applications ranging from video surveillance to autonomous driving. Despite achieving high performance, it is still largely unknown how well existing detectors generalize to unseen data. This is important because a practical detector should be ready to use in various scenarios in applications. To this end, we conduct a comprehensive study in this paper, using a general principle of direct cross-dataset evaluation. Through this study, we find that existing state-of-the-art pedestrian detectors, though perform quite well when trained and tested on the same dataset, generalize poorly in cross dataset evaluation. We demonstrate that there are two reasons for this trend. Firstly, their designs (e.g. anchor settings) may be biased towards popular benchmarks in the traditional single-dataset training and test pipeline, but as a result largely limit their generalization capability. Secondly, the training source is generally not dense in pedestrians and diverse in scenarios. 
Under direct cross-dataset evaluation, surprisingly, we find that a general purpose object detector, without pedestrian-tailored adaptation in design, generalizes much better compared to existing state-of-the-art pedestrian detectors. Furthermore, we illustrate that diverse and dense datasets, collected by crawling the web, serve to be an efficient source of pre-training for pedestrian detection. Accordingly, we propose a progressive training pipeline and find that it works well for autonomous-driving oriented pedestrian detection. Consequently, the study conducted in this paper suggests that more emphasis should be put on cross-dataset evaluation for the future design of generalizable pedestrian detectors. Code and models can be accessed at \url{https://github.com/hasanirtiza/Pedestron}.

\end{abstract}

==> sections/discussion.tex <==
\section{Discussion and Analysis} \label{sec:disc}
\subsection{Effect of Fine-tuning on Target Data}

With study presented in section \ref{sec:general-cap}, we find that existing methods may overfit on a single dataset, and so we suggest to put more emphasis on cross-dataset evaluation for a new way of benchmarking. However, to align to the previously established evaluation protocol on single dataset and compare to the existing state of the art, we conduct an additional study on fine-tuning our above models on target data. Experimental results show that, with progressively trained and generalizable baseline models, it is relatively more easy to adapt to new datasets by fine-tuning, and further performance gain can be achieved.

%  Therefore, we investigated the effect of pre-training on a large scale autonomous driving dataset along with fine-tuning on target dataset as reported in Table \ref{tab:finetune}. \emph{A} $\rightarrow$ \emph{B} refers to pre-training on \emph{A} and fine-tuning on the target dataset \emph{B}. Visible improvements can be seen in the case of \caltech{}, which resonates with our previous findings that due to low-resolution and sparse annotation, pre-training on \ecpa{} or \cityperson{} boosts the performances on \caltech{}. 
%  Importantly, in the case of \cityperson{}, the pre-training on \ecpa{} brings improvement of nearly 2$\%$ of \LMR{}, as discussed above, \ecpa{} brings density, both in terms of number of pedestrians and pedestrians per frame. Conversely, due to relative smaller size, the pre-training on \cityperson{} does not bring any improvements on \ecpa{}.
 
 

% On much challenging autonomous driving datasets such as \cityperson{} and \ecp{} as shown in Table \ref{tab:icon-ch-wider}, mere pre-training on diverse and dense pedestrian datasets does not result in any improvements compared to second and fifth row of Table \ref{tab:cross-cp-ecp-cal}. Since \crowdhuman{} and \widerperson{} though larger in diversity and density still are relatively under-represented in terms of only autonomous driving scenes, therefore fine-tuning on the target dataset is a necessity. 
% In Table \ref{tab:icon-finetune}, we present results of pre-training on a dataset and fine-tuning on the target dataset. \emph{A} $\rightarrow$ \emph{B} refers to pre-training on \emph{A} and fine-tuning on the target dataset \emph{B}. 
% Table \ref{tab:icon-finetune} shows that pre-training on a web-crawled dataset, with large diversity and density and subsequently fine-tuned on the target dataset provides significant improvements over only pre-training on the autonomous driving datasets and fine-tuning on the target datasets. 
% Improvements are consistent across all datasets and on all occlusion and size settings. 
% In comparison with Table \ref{tab:finetune}, where pre-training is done on autonomous driving datasets, improvement across all dataset (taking the best cases) are $3.3\%$, $0.4\%$ and $2.4\%$ of \LMR{} percentage points on \caltecha{}{}, \cityperson{} and \ecp{}, respectively. 
% Interestingly, \widerperson{} appears to be slightly better source of pre-training than \crowdhuman{} since it contains more images of autonomous driving scenes. 
% Finally, in Table \ref{tab:icon-finetune2}, starting with a pre-training on the web-crawled dataset, we fine-tuned our model on the largest autonomous driving dataset \ecp{} and subsequently fine-tuning on the target dataset. We refer to this as our \emph{progressive training pipeline}, results show that the best performances are achieved by using this training pipeline. Significant improvements across all datasets and under all evaluation settings can be observed using the progressive training pipeline where we eventually fine-tune on the target domain. Particularly, in comparison with \ref{tab:icon-finetune}, progressive pipeline improves upon previous performances on \textit{reasonable}/\textit{heavy} subsets of \emph{CityPersons} dataset by 1.6$\%$/14.4$\%$ and on \emph{Caltech} by 0.7$\%$/5.0$\%$ in terms of log average miss rate (\LMR{}) points.

% Note that though fine-tuning to a very specific domain does improve the performance on that domain, it requires human effort to annotate more data from that domain, and the obtained model may only be useful on that domain but on longer be generally effective on other domains. Therefore, to avoid human annotation in deployment of the detector and to keep a general model that can be applied to most scenarios, we still prefer to train a universal model and validate it by cross-dataset evaluation without adaptation on target data.






















% \begin{table}[t]
% %\parbox{.5\linewidth}{
% \centering
% \caption{Investigating  the performance of embedded vision model, when pre-trained on diverse and dense datasets.}
% \label{tab:mobileNet}
%   \resizebox{0.98\linewidth}{!}{
% \begin{tabular}{l|c|c|c}
% \hline
% Training             & Reasonable & Small & Heavy \\ \hline
% CP    & 12.0     & 15.3     & 47.8 \\ \hline
% CrowdHuman$\rightarrow$CP  & 11.8   & 14.6   & 41.6   \\ \hline
% CrowdHuman$\rightarrow$ECP$\rightarrow$CP    &    10.9 & 14.4     &  44.6\\ \hline
% Wider Pedestrian$\rightarrow$CP  & 11.7     & 14.9   & 45.6   \\ \hline
% Wider Pedestrian$\rightarrow$ECP$\rightarrow$CP    & \textbf{10.1}    & \textbf{11.9}    & \textbf{35.4} \\ \hline
% \end{tabular}
% }
% %}
% \end{table}

% \begin{table}[t]

% %\parbox{.5\linewidth}{
% \centering
% \caption{WiderPerson split.}
% \label{tab:mobileNet}
% %\resizebox{0.98\linewidth}{!}{
% \begin{tabular}{l|c|c|c}
% \hline
% Training             & Reasonable & Small & Heavy \\ \hline

% Wider-AD$\rightarrow$CP  &   &    &    \\ \hline
% Wider-AD$\rightarrow$ECP$\rightarrow$CP    &     &      & \\ \hline
% Wider-SUR$\rightarrow$CP  &      &    &   \\ \hline
% Wider-SUR$\rightarrow$ECP$\rightarrow$CP    &    &      & \\ \hline
% \end{tabular}
% %}
% %}
% \end{table}



% \subsection{Application Oriented Models}

% In many pedestrian detection applications, the size and computational cost of models is constrained.
% We experiment with a small and light-weight model MobileNet \cite{howard2017mobilenets}, which is designed for mobile and embedded vision applications, to investigate if the performance improvements hold true.
% %We investigated a light-weight mobile and embedded vision application oriented model MobileNet \cite{howard2017mobilenets}, providing fast speed and fewer hyper-parameters, thus tailor-made for practical applications. 
% Table \ref{tab:mobileNet} shows results on \cityperson{} using \mobnet{} as a backbone network architecture into our baseline. 
% Intuitively, \mobnet{} performs worse than the HRNet \cite{wang2019deep}. 
% However, in the case of \mobnet{} as well, we see pre-training on \crowdhuman{} and fine-tuning on \cityperson{} improves the performance of the \mobnet{}. 
% Subsequently, we pre-train (3rd row) \mobnet{} on \crowdhuman{} and \ecp{} before fine-tuning on \cityperson{}. 
% Improvement of nearly 1$\%$ of \LMR{} can be observed. 
% Furthermore, we replaced \crowdhuman{} with \widerperson{} as the initial source of pre-training. Improvement over the baseline (1st row) can be observed (4th row). 
% Importantly, in the last row of Table \ref{tab:mobileNet}, largest gain can be observed. 
% This is consistent with our previous finding reported in Table \ref{tab:icon-finetune2}, \widerperson{} is a better source of pre-training than \crowdhuman{}, since it has images of autonomous driving scenes as well making it more diverse than \crowdhuman{}. 
% Interestingly, in the case of \crowdhuman{} and \widerperson{}, even with a light-weight architecture, our baseline outperformed state-of-the-art pedestrian detector CSP \cite{Liu2018DBC}. 
% In summary, even with a light weight back-bone architecture, by pre-training on diverse and dense datasets, \mobnet{} outperformed previous best performing method on \cityperson{}, i.e. CSP \cite{Liu2018DBC}.  


% \subsection{Failure Cases}

% \begin{figure}[tbh]
% \begin{subfigure}{0.19\textwidth}
%   \centering
%   % include first image
%   \includegraphics[height=0.19\textheight]{images/fp-easy/amsterdam_01217.jpg}
%   \caption{}
%   \label{fig:failures:fp:easy1}
% \end{subfigure}
% \bigskip % force a bit of vertical whitespace
% \begin{subfigure}{0.16\textwidth}
%   \centering
%   \includegraphics[height=0.19\textheight]{images/fp-easy/barcelona_01488.jpg}  
%   \caption{}
%   \label{fig:failures:fp:easy2}
% \end{subfigure}
% \begin{subfigure}{0.23\textwidth}
%   \centering
%   % include first image
%   \includegraphics[height=0.19\textheight]{images/fp-anno/barcelona_01504.jpg}
%   \caption{}
%   \label{fig:failures:fp:anno1}
% \end{subfigure}
% \begin{subfigure}{0.23\textwidth}
%   \centering
%   % include first image
%   \includegraphics[height=0.19\textheight]{images/fp-anno/bologna_01299.jpg}
%   \caption{}
%   \label{fig:failures:fp:anno2}
% \end{subfigure}
% \begin{subfigure}{.15\textwidth}
%   \centering
%   % include first image
%   \includegraphics[height=0.19\textheight]{images/fp-anno/bologna_01364.jpg}
%   \caption{}
%   \label{fig:failures:fp:anno3}
% \end{subfigure}

% \vspace{-0.25cm}
% \begin{subfigure}{0.11\textwidth}
%   \centering
%   % include first image
%   \includegraphics[height=0.19\textheight]{images/fn-easy/amsterdam_01140.jpg}  
%   \caption{}
%   \label{fig:failures:fn:1}
% \end{subfigure}
% \bigskip % force a bit of vertical whitespace
% \begin{subfigure}{0.21\textwidth}
%   \centering
%   \includegraphics[height=0.19\textheight]{images/fn-easy/barcelona_01444.jpg}  
%   \caption{}
%   \label{fig:failures:fn:2}
% \end{subfigure}
% \begin{subfigure}{0.21\textwidth}
%   \centering
%   % include first image
%   \includegraphics[height=0.19\textheight]{images/fn-easy/barcelona_01283.jpg}  
%   \caption{}
%   \label{fig:failures:fn:3}
% \end{subfigure}
% \begin{subfigure}{0.19\textwidth}
%   \centering
%   % include first image
%   \includegraphics[height=0.19\textheight]{images/fn-easy/barcelona_01336.jpg}  
%   \caption{}
%   \label{fig:failures:fn:4}
% \end{subfigure}
% \begin{subfigure}{.15\textwidth}
%   \centering
%   % include first image
%   \includegraphics[height=0.19\textheight]{images/fn-easy/basel_00692.jpg}  
%   \caption{}
%   \label{fig:failures:fn:5}
% \end{subfigure}
% \vspace{-0.6cm}
% \caption{Failure cases for Cascade R-CNN\textsuperscript{$\dagger$} on EuroCityPersons at 0.1 false positive per image.
% Top row: False positives. Bottom row: False negatives.}
% \label{fig:failures}
% \end{figure}


% % \todo{selected errors: \url{https://drive.google.com/open?id=1ELtQ-4_8CDPRtSG-08wDJVpifb4dGnZU}}
% Most of the errors of our best model are quite challenging cases either due to large occlusion, small size of the pedestrian, low illumination and/or the presence of another pedestrian in the vicinity, which leads to the bounding box of the pedestrian being deleted as has been reported previously \cite{braun2018eurocity}.
% In Fig.\ref{fig:failures}, we shows some examples of the easiest (for a human) false negatives (FN) and false positives (FP) samples at 0.1 FP per image.
% Some FPs, Fig.\ref{fig:failures:fp:easy1}-\ref{fig:failures:fp:easy2}, are due to depictions of people in pictures, and due to shadows and objects which slightly resemble a pedestrian but the model fails to correctly classify them.
% We also show few false positives in Fig.\ref{fig:failures:fp:anno1}-\ref{fig:failures:fp:anno3}, which are due to annotation mistakes.
% Even though, most false negatives are difficult even for a human, the model nevertheless sometimes fails to detect relatively easy (large, non-occluded) pedestrians and the cause of many of these failure is not obvious.
% Fig.\ref{fig:failures:fn:1}-\ref{fig:failures:fn:5} shows some of these cases.

% Most of the failures of the model are extremely challenging cases, where it is difficult to determine whether the false positives (FPs) are actually a pedestrian and the annotators have missed them or the model has made a mistake and cases where the shadow or background objects look similar to a pedestrian.
% Similarly, most of the False negatives (FNs) are pedestrians which are heavily occluded, with only a small part of pedestrian is visible.

% Even though most of the errors are very challenging cases, there are nevertheless some easy but uncommon cases where the model fails to detect pedestrians, e.g person sitting in a car, on a bench, or in a construction vehicle, etc. or detects pedestrians in background, e.g. picture on the side of a vehicle, etc.

% There are also some cases where the pedestrian is un-occluded and quite large, but the model still fails, so even though the proposed model improves performance considerably, it nevertheless can fail for some relatively easy cases.



==> sections/discussion_old.tex <==
\section{Discussion and Analysis} \label{sec:disc}
\subsection{Effect of Fine-tuning on Target Data}

With study presented in section \ref{sec:general-cap}, we find that existing methods may overfit on a single dataset, and so we suggest to put more emphasis on cross-dataset evaluation for a new way of benchmarking. However, to align to the previously established evaluation protocol on single dataset and compare to the existing state of the art, we conduct an additional study on fine-tuning our above models on target data. Experimental results show that, with progressively trained and generalizable baseline models, it is relatively more easy to adapt to new datasets by fine-tuning, and further performance gain can be achieved.

 Therefore, we investigated the effect of pre-training on a large scale autonomous driving dataset along with fine-tuning on target dataset as reported in Table \ref{tab:finetune}. \emph{A} $\rightarrow$ \emph{B} refers to pre-training on \emph{A} and fine-tuning on the target dataset \emph{B}. Visible improvements can be seen in the case of \caltech{}, which resonates with our previous findings that due to low-resolution and sparse annotation, pre-training on \ecpa{} or \cityperson{} boosts the performances on \caltech{}. 
 Importantly, in the case of \cityperson{}, the pre-training on \ecpa{} brings improvement of nearly 2$\%$ of \LMR{}, as discussed above, \ecpa{} brings density, both in terms of number of pedestrians and pedestrians per frame. Conversely, due to relative smaller size, the pre-training on \cityperson{} does not bring any improvements on \ecpa{}.
 
 
 \begin{table}[tb]
\centering
\caption{Showing how well CityPersons (CP) and ECP are as the source of pre-training.}
\label{tab:finetune}
\begin{tabular}{l|c|c|c}
\hline
Training             & Reasonable & Small & Heavy \\ \hline
CP$\rightarrow$Caltech    & 5.9   & 8.6      & 27.0 \\ \hline
ECP$\rightarrow$Caltech    &  5.7 & 7.7      & 26.8  \\ \hline
CP$\rightarrow$ECP    &  6.8   & 12.3     & 33.0\\ \hline
ECP$\rightarrow$CP  & 9.59   &    11.04 & 36.0  \\ \hline
\end{tabular}
\end{table}
 
On much challenging autonomous driving datasets such as \cityperson{} and \ecp{} as shown in Table \ref{tab:icon-ch-wider}, mere pre-training on diverse and dense pedestrian datasets does not result in any improvements compared to second and fifth row of Table \ref{tab:cross-cp-ecp-cal}. Since \crowdhuman{} and \widerperson{} though larger in diversity and density still are relatively under-represented in terms of only autonomous driving scenes, therefore fine-tuning on the target dataset is a necessity. 
In Table \ref{tab:icon-finetune}, we present results of pre-training on a dataset and fine-tuning on the target dataset. \emph{A} $\rightarrow$ \emph{B} refers to pre-training on \emph{A} and fine-tuning on the target dataset \emph{B}. 
Table \ref{tab:icon-finetune} shows that pre-training on a web-crawled dataset, with large diversity and density and subsequently fine-tuned on the target dataset provides significant improvements over only pre-training on the autonomous driving datasets and fine-tuning on the target datasets. 
Improvements are consistent across all datasets and on all occlusion and size settings. 
In comparison with Table \ref{tab:finetune}, where pre-training is done on autonomous driving datasets, improvement across all dataset (taking the best cases) are $3.3\%$, $0.4\%$ and $2.4\%$ of \LMR{} percentage points on \caltecha{}{}, \cityperson{} and \ecp{}, respectively. 
Interestingly, \widerperson{} appears to be slightly better source of pre-training than \crowdhuman{} since it contains more images of autonomous driving scenes. 
Finally, in Table \ref{tab:icon-finetune2}, starting with a pre-training on the web-crawled dataset, we fine-tuned our model on the largest autonomous driving dataset \ecp{} and subsequently fine-tuning on the target dataset. We refer to this as our \emph{progressive training pipeline}, results show that the best performances are achieved by using this training pipeline. Significant improvements across all datasets and under all evaluation settings can be observed using the progressive training pipeline where we eventually fine-tune on the target domain. Particularly, in comparison with \ref{tab:icon-finetune}, progressive pipeline improves upon previous performances on \textit{reasonable}/\textit{heavy} subsets of \emph{CityPersons} dataset by 1.6$\%$/14.4$\%$ and on \emph{Caltech} by 0.7$\%$/5.0$\%$ in terms of log average miss rate (\LMR{}) points.

Note that though fine-tuning to a very specific domain does improve the performance on that domain, it requires human effort to annotate more data from that domain, and the obtained model may only be useful on that domain but on longer be generally effective on other domains. Therefore, to avoid human annotation in deployment of the detector and to keep a general model that can be applied to most scenarios, we still prefer to train a universal model and validate it by cross-dataset evaluation without adaptation on target data.


\begin{table}[tb]
\centering
\caption{Illustrating how our baseline behave with fine-tuning on the target dataset when CrowdHuman and Wider Pedestrian are used as a source of pre-training.}
\label{tab:icon-finetune}
 \resizebox{0.98\linewidth}{!}{
\begin{tabular}{l|c|c|c}
\hline
Training             & Reasonable & Small & Heavy \\ \hline
CrowdHuman$\rightarrow$Caltech    &  2.7    &  10.9     & 31.0  \\ \hline
Wider Pedestrian$\rightarrow$Caltech    & \textbf{2.4}  &   \textbf{9.8}   & \textbf{30.7}  \\ \hline
\hline
CrowdHuman$\rightarrow$CP    &  9.2   & 14.7      & 38.02\\ \hline
Wider Pedestrian$\rightarrow$CP  &  \textbf{9.1}  & \textbf{11.0}     & \textbf{34.4}   \\ \hline
\hline
CrowdHuman$\rightarrow$ECP    &  4.5   &   9.3   & 23.0 \\ \hline
Wider Pedestrian$\rightarrow$ECP  &  \textbf{4.4}    &  \textbf{9.1}   & \textbf{21.3}  \\ \hline
\end{tabular}
}
\end{table}

\begin{table}[tb]
\centering
\caption{Showing the effect of fine-tuning in a cascaded manner.}
\label{tab:icon-finetune2}
 \resizebox{0.99\linewidth}{!}{
\begin{tabular}{l|c|c|c}
\hline
Training             & Reasonable & Small & Heavy \\ \hline
ECP$\rightarrow$Caltech    &    5.7 & 7.7     & 26.8  \\ \hline
CrowdHuman$\rightarrow$ECP$\rightarrow$Caltech    & 2.2     &   8.1   & 30.7 \\ \hline
Wider Pedestrian$\rightarrow$ECP$\rightarrow$Caltech    &  \textbf{1.7}  & \textbf{7.2}     & \textbf{25.7}\\ \hline
\hline
ECP$\rightarrow$CP  & 9.5     & 11.0   & 36.0  \\ \hline
CrowdHuman$\rightarrow$ECP$\rightarrow$CP  & 8.0     & 8.5   & 27.0  \\ \hline
Wider Pedestrian$\rightarrow$ECP$\rightarrow$CP  & \textbf{7.5}     & \textbf{8.0}    & \textbf{28.0}  \\ \hline
\end{tabular}
}
\end{table}



\subsection{Comparison with Current State-of-the-Art}
In this section we present a comparative analysis of state-of-the-art of pedestrian detection. For our comparative analysis, we choose the best performing pedestrian detectors on \caltech{} and \cityperson{}. The underlying goal is to illustrate how well our baseline performs when it is fine-tune on the target dataset.
We refer to the best performing baseline presented in Table \ref{tab:icon-finetune2} as \textbf{\emph{Cascade R-CNN}}\textsuperscript{$\dagger$}. 
Table \ref{tab:Caltech-SOTA} shows that \textbf{\emph{Cascade R-CNN}}\textsuperscript{$\dagger$} achieves 1.76 \LMR{} on \caltech{}, outperforming previous best by a margin of $3.24\%$ of \LMR{}. 
This performance is approaching \emph{human-baseline} (0.88) \cite{zhang2016far} on \caltech{} .
Moreover, we report similar improvement over the previous state-of-the-art on \cityperson{} benchmark. \textbf{\emph{Cascade R-CNN's}}\textsuperscript{$\dagger$} performance is $3.5\%$ \LMR{} better than CSP \cite{Liu2018DBC}. 
Finally, on \ecp{} we report an improvements of $1.8\%$ \LMR{} over Faster R-CNN \cite{ren2015faster}. 
Similar performance improvements are achieved on other subsets of all these three datasets, with the performance improvement of more than 50\% for the most challenging subsets, \textit{Heavy} and \textit{small}.
This consistent improvement over all datasets illustrates the robustness of the \textbf{\emph{Cascade R-CNN}}\textsuperscript{$\dagger$}, as it significantly outperform previous state-of-the-art.

\begin{table}[tb]
\centering
\caption{Comparison with state-of-the-art on Caltech.}
\label{tab:Caltech-SOTA}
%  \resizebox{0.98\linewidth}{!}{
\begin{tabular}{l|c|c|c}
\hline
Method         & Reasonable & Heavy & All  \\ \hline
DeepParts\cite{tian2015deep}       & 11.89      & 60.42 & --   \\ \hline
CompactACT-Deep\cite{cai2015learning} & 9.2        & --    & --   \\ \hline
FRCNN\cite{zhang2017citypersons}           & 8.7        & 53.1  & 62.6 \\ \hline
RPN +BF\cite{zhang2016faster}         & 7.3        & 54.6  & 59.9 \\ \hline
ALFNet\cite{liu2018learning}          & 6.1        & 51.0  & 59.1 \\ \hline
Hyper Learner\cite{mao2017can}   & 5.5        & 48.7  & 61.5 \\ \hline
Rep Loss\cite{wang2018repulsion}        & 5.0        & 47.9  & 59.0 \\ \hline
CSP\cite{Liu2018DBC}   & 5.8        & 46.6  & 57.7 \\ \hline
\textbf{\emph{Cascade R-CNN}}\textsuperscript{$\dagger$}        & \textbf{1.7}        & \textbf{25.7}  &\textbf{ 27.4} \\ \hline
\end{tabular}
%}
\end{table}

\begin{table}[]
\centering
\caption{Comparison with state-of-the-art on ECP. The results are evaluated on the testing set.}
\label{tab:ECP-SOTA}
%  \resizebox{0.98\linewidth}{!}{
\begin{tabular}{l|c|c|c}
\hline
Method             & Reasonable & Small & Heavy \\ \hline
Faster R-CNN    & 7.3  & 16.6     & 52.0 \\ \hline
YOLOv3    &  8.5 & 17.8     & 37.0\\ \hline
SSD &  10.5 & 20.5   & 42.0 \\ \hline
\textbf{\emph{Cascade R-CNN}}\textsuperscript{$\dagger$} & \textbf{5.5}    & \textbf{11.7}   & \textbf{26.1} \\ \hline
\end{tabular}
%}
\end{table}



\begin{table*}[ht]
\begin{center}
\caption{Comparison with state-of-the-art on CityPersons.}
\label{tab:City-SOTA}
\resizebox{.999\textwidth}{!}{
\begin{tabular}{c|c|c|c c c|c c c|c}
\hline
Method & Backbone & Reasonable & Heavy*  & Partial & Bare & Small & Medium & Large & Test Time\\
\hline
\hline
FRCNN\cite{zhang2017citypersons} & VGG-16 & 15.4 & - & - & - & 25.6 & 7.2 & 7.9 & -\\
\hline
RetinaNet \cite{lin2017focal}  & ResNet-50 & 15.6 & 49.9 & - & - & - & - & - & -\\
\hline
CornerNet \cite{Law_2018_ECCV} & Hourglass-54 & 21.0 & 56.0 & - & - & - & - & - & -\\
\hline
FRCNN+Seg\cite{zhang2017citypersons} & VGG-16 & 14.8 & - & - & - & 22.6 & 6.7 & 8.0 & -\\
\hline
OR-CNN\cite{zhang2018occlusion} & VGG-16 & 12.8 & 55.7 & 15.3 & 6.7 & - & - & - & -\\
\hline
RepLoss\cite{wang2018repulsion} & ResNet-50 & 13.2 & 56.9 & 16.8 & 7.6 & - & - & -& -\\
\hline
TLL\cite{song2018small} & ResNet-50 & 15.5 & 53.6 & 17.2 & 10.0 & - & - & -& -\\
\hline
TLL+MRF\cite{song2018small} & ResNet-50 & 14.4 & 52.0 & 15.9 & 9.2 & - & - & -& -\\
\hline
ALFNet\cite{liu2018learning} & ResNet-50 & 12.0 & 51.9 & 11.4 & 8.4 & 19.0 & 5.7 & 6.6 & 0.27s/img\\
\hline
CSP\cite{Liu2018DBC} & ResNet-50 & {11.0} & 49.3 & 10.4 & {7.3} & {16.0} & {3.7} & {6.5}& 0.33s/img\\
\hline
\textbf{\emph{Cascade R-CNN}}\textsuperscript{$\dagger$} & HRNet & \textbf{{7.5}} & \textbf{{33.9}} & \textbf{5.7} & \textbf{6.2} & \textbf{8.0} & \textbf{3.0} & \textbf{4.3}  & 0.33s/img\\
\hline
\end{tabular}
}
\end{center}

\end{table*}










\begin{table}[t]
%\parbox{.5\linewidth}{
\centering
\caption{Investigating  the performance of embedded vision model, when pre-trained on diverse and dense datasets.}
\label{tab:mobileNet}
  \resizebox{0.98\linewidth}{!}{
\begin{tabular}{l|c|c|c}
\hline
Training             & Reasonable & Small & Heavy \\ \hline
CP    & 12.0     & 15.3     & 47.8 \\ \hline
CrowdHuman$\rightarrow$CP  & 11.8   & 14.6   & 41.6   \\ \hline
CrowdHuman$\rightarrow$ECP$\rightarrow$CP    &    10.9 & 14.4     &  44.6\\ \hline
Wider Pedestrian$\rightarrow$CP  & 11.7     & 14.9   & 45.6   \\ \hline
Wider Pedestrian$\rightarrow$ECP$\rightarrow$CP    & \textbf{10.1}    & \textbf{11.9}    & \textbf{35.4} \\ \hline
\end{tabular}
}
%}
\end{table}

% \begin{table}[t]

% %\parbox{.5\linewidth}{
% \centering
% \caption{WiderPerson split.}
% \label{tab:mobileNet}
% %\resizebox{0.98\linewidth}{!}{
% \begin{tabular}{l|c|c|c}
% \hline
% Training             & Reasonable & Small & Heavy \\ \hline

% Wider-AD$\rightarrow$CP  &   &    &    \\ \hline
% Wider-AD$\rightarrow$ECP$\rightarrow$CP    &     &      & \\ \hline
% Wider-SUR$\rightarrow$CP  &      &    &   \\ \hline
% Wider-SUR$\rightarrow$ECP$\rightarrow$CP    &    &      & \\ \hline
% \end{tabular}
% %}
% %}
% \end{table}



% \subsection{Application Oriented Models}

% In many pedestrian detection applications, the size and computational cost of models is constrained.
% We experiment with a small and light-weight model MobileNet \cite{howard2017mobilenets}, which is designed for mobile and embedded vision applications, to investigate if the performance improvements hold true.
% %We investigated a light-weight mobile and embedded vision application oriented model MobileNet \cite{howard2017mobilenets}, providing fast speed and fewer hyper-parameters, thus tailor-made for practical applications. 
% Table \ref{tab:mobileNet} shows results on \cityperson{} using \mobnet{} as a backbone network architecture into our baseline. 
% Intuitively, \mobnet{} performs worse than the HRNet \cite{wang2019deep}. 
% However, in the case of \mobnet{} as well, we see pre-training on \crowdhuman{} and fine-tuning on \cityperson{} improves the performance of the \mobnet{}. 
% Subsequently, we pre-train (3rd row) \mobnet{} on \crowdhuman{} and \ecp{} before fine-tuning on \cityperson{}. 
% Improvement of nearly 1$\%$ of \LMR{} can be observed. 
% Furthermore, we replaced \crowdhuman{} with \widerperson{} as the initial source of pre-training. Improvement over the baseline (1st row) can be observed (4th row). 
% Importantly, in the last row of Table \ref{tab:mobileNet}, largest gain can be observed. 
% This is consistent with our previous finding reported in Table \ref{tab:icon-finetune2}, \widerperson{} is a better source of pre-training than \crowdhuman{}, since it has images of autonomous driving scenes as well making it more diverse than \crowdhuman{}. 
% Interestingly, in the case of \crowdhuman{} and \widerperson{}, even with a light-weight architecture, our baseline outperformed state-of-the-art pedestrian detector CSP \cite{Liu2018DBC}. 
% In summary, even with a light weight back-bone architecture, by pre-training on diverse and dense datasets, \mobnet{} outperformed previous best performing method on \cityperson{}, i.e. CSP \cite{Liu2018DBC}.  


% \subsection{Failure Cases}

% \begin{figure}[tbh]
% \begin{subfigure}{0.19\textwidth}
%   \centering
%   % include first image
%   \includegraphics[height=0.19\textheight]{images/fp-easy/amsterdam_01217.jpg}
%   \caption{}
%   \label{fig:failures:fp:easy1}
% \end{subfigure}
% \bigskip % force a bit of vertical whitespace
% \begin{subfigure}{0.16\textwidth}
%   \centering
%   \includegraphics[height=0.19\textheight]{images/fp-easy/barcelona_01488.jpg}  
%   \caption{}
%   \label{fig:failures:fp:easy2}
% \end{subfigure}
% \begin{subfigure}{0.23\textwidth}
%   \centering
%   % include first image
%   \includegraphics[height=0.19\textheight]{images/fp-anno/barcelona_01504.jpg}
%   \caption{}
%   \label{fig:failures:fp:anno1}
% \end{subfigure}
% \begin{subfigure}{0.23\textwidth}
%   \centering
%   % include first image
%   \includegraphics[height=0.19\textheight]{images/fp-anno/bologna_01299.jpg}
%   \caption{}
%   \label{fig:failures:fp:anno2}
% \end{subfigure}
% \begin{subfigure}{.15\textwidth}
%   \centering
%   % include first image
%   \includegraphics[height=0.19\textheight]{images/fp-anno/bologna_01364.jpg}
%   \caption{}
%   \label{fig:failures:fp:anno3}
% \end{subfigure}

% \vspace{-0.25cm}
% \begin{subfigure}{0.11\textwidth}
%   \centering
%   % include first image
%   \includegraphics[height=0.19\textheight]{images/fn-easy/amsterdam_01140.jpg}  
%   \caption{}
%   \label{fig:failures:fn:1}
% \end{subfigure}
% \bigskip % force a bit of vertical whitespace
% \begin{subfigure}{0.21\textwidth}
%   \centering
%   \includegraphics[height=0.19\textheight]{images/fn-easy/barcelona_01444.jpg}  
%   \caption{}
%   \label{fig:failures:fn:2}
% \end{subfigure}
% \begin{subfigure}{0.21\textwidth}
%   \centering
%   % include first image
%   \includegraphics[height=0.19\textheight]{images/fn-easy/barcelona_01283.jpg}  
%   \caption{}
%   \label{fig:failures:fn:3}
% \end{subfigure}
% \begin{subfigure}{0.19\textwidth}
%   \centering
%   % include first image
%   \includegraphics[height=0.19\textheight]{images/fn-easy/barcelona_01336.jpg}  
%   \caption{}
%   \label{fig:failures:fn:4}
% \end{subfigure}
% \begin{subfigure}{.15\textwidth}
%   \centering
%   % include first image
%   \includegraphics[height=0.19\textheight]{images/fn-easy/basel_00692.jpg}  
%   \caption{}
%   \label{fig:failures:fn:5}
% \end{subfigure}
% \vspace{-0.6cm}
% \caption{Failure cases for Cascade R-CNN\textsuperscript{$\dagger$} on EuroCityPersons at 0.1 false positive per image.
% Top row: False positives. Bottom row: False negatives.}
% \label{fig:failures}
% \end{figure}


% % \todo{selected errors: \url{https://drive.google.com/open?id=1ELtQ-4_8CDPRtSG-08wDJVpifb4dGnZU}}
% Most of the errors of our best model are quite challenging cases either due to large occlusion, small size of the pedestrian, low illumination and/or the presence of another pedestrian in the vicinity, which leads to the bounding box of the pedestrian being deleted as has been reported previously \cite{braun2018eurocity}.
% In Fig.\ref{fig:failures}, we shows some examples of the easiest (for a human) false negatives (FN) and false positives (FP) samples at 0.1 FP per image.
% Some FPs, Fig.\ref{fig:failures:fp:easy1}-\ref{fig:failures:fp:easy2}, are due to depictions of people in pictures, and due to shadows and objects which slightly resemble a pedestrian but the model fails to correctly classify them.
% We also show few false positives in Fig.\ref{fig:failures:fp:anno1}-\ref{fig:failures:fp:anno3}, which are due to annotation mistakes.
% Even though, most false negatives are difficult even for a human, the model nevertheless sometimes fails to detect relatively easy (large, non-occluded) pedestrians and the cause of many of these failure is not obvious.
% Fig.\ref{fig:failures:fn:1}-\ref{fig:failures:fn:5} shows some of these cases.

% Most of the failures of the model are extremely challenging cases, where it is difficult to determine whether the false positives (FPs) are actually a pedestrian and the annotators have missed them or the model has made a mistake and cases where the shadow or background objects look similar to a pedestrian.
% Similarly, most of the False negatives (FNs) are pedestrians which are heavily occluded, with only a small part of pedestrian is visible.

% Even though most of the errors are very challenging cases, there are nevertheless some easy but uncommon cases where the model fails to detect pedestrians, e.g person sitting in a car, on a bench, or in a construction vehicle, etc. or detects pedestrians in background, e.g. picture on the side of a vehicle, etc.

% There are also some cases where the pedestrian is un-occluded and quite large, but the model still fails, so even though the proposed model improves performance considerably, it nevertheless can fail for some relatively easy cases.



==> sections/related_work.tex <==
\section{Related Work} \label{sec:prev}

\noindent\textbf{Pedestrian detection.} Before the emergence of CNNs, a common  way to address this problem was to exhaustively operate in a sliding window manner over all possible locations and scales, inspired from Viola and Jones \cite{viola2004robust}. 
Dalal and Triggs in their landmark pedestrian detection work \cite{dalal2005histograms} proposed Histogram of Oriented Gradients (HOG) feature descriptor for representing pedestrians.
Dollar et al \cite{dollar2014fast}, proposed ACF, where the key idea was to use features across multiple channels. 
Similarly, \cite{zhang2017citypersons,paisitkriangkrai2014strengthening}, used filtered channel features and low-level visual features along with spatial pooling respectively for pedestrian detection. %
However, the use of engineered features meant very limited generalization ability and limited performance.    

In recent years, Convolutional Neural Networks (CNNs) have become the dominant paradigm in generic object detection \cite{ren2015faster,he2017mask,sun2018fishnet,liu2016ssd}.
The same trend is also true for the pedestrian detection \cite{angelova2015real,hosang2015taking,cai2015learning}. 
Some of the pioneer works for CNN based pedestrian detection \cite{hosang2015taking,zhang2016far} used R-CNN framework \cite{girshick2014rich}, which is still the most popular framework.
RPN+BF \cite{zhang2016faster} was the first work to use Region Proposal Network (RPN); it used boosted forest for improving pedestrian detection performance.
This work also pointed out some problems in the underlying classification branch of Faster RCNN \cite{ren2015faster}, namely that the resolution of the feature maps and class-imbalance. 
However, RPN+BF despite achieving good performances had a shortcoming of not being optimized end-to-end. After the initial works, Faster RCNN \cite{ren2015faster} became most popular framework with wide range of literature deploying it for pedestrian detection \cite{zhou2018bi,zhang2017citypersons,cai2016unified,brazil2017illuminating,mao2017can}. 

Some of the recent state-of-the-art pedestrian detectors include ALF \cite{liu2018learning}, CSP \cite{Liu2018DBC} and MGAN \cite{pang2019maskguided}.
ALF \cite{liu2018learning} is based on Single Shot MultiBox Detector (SSD) \cite{liu2016ssd}, it stacks together multiple predictors to learn a better detection from default anchor boxes.
MGAN \cite{pang2019maskguided} uses the segmentation mask of the visible region of a pedestrian to guide the network attention and improve performance on occluded pedestrians.
CSP is an anchor-less fully convolutional detector, which utilizes concatenated feature maps for predicting pedestrians.
%CSP defined new state-of-the-art in pedestrian detection and although, our work is detector agnostic in this work we use CSP as our baseline detector.

\iffalse
Occlusion stands as one of the major problems in pedestrian detection. 
In the past, engineered selection of human parts were used to reason over, in order to handle occlusion \cite{wu2005detection,shet2007bilattice,enzweiler2010multi,duan2010structura,ouyang2012discriminative,tian2015deep,ouyang2013joint,zhou2016learning,zhou2017multi,noh2018improving,zhoudiscriminative,mathias2013handling,chu2013tracking,lee2014driving}. 
Since, the selection of human parts were hand-crafted, this resulted in limited generalization ability of these approaches. Recently, Bi-Box regression \cite{zhou2018bi}, extended the architecture of Faster R-CNN by adding an occlusion branch, which learnt features only for visible part of a pedestrian.  Another work \cite{lin2018graininess}, addressed occlusion handling by incorporating extra fine-grained information into low resolution feature maps to make it more robust to occlusion. An occlusion-aware R-CNN is proposed in \cite{zhang2018occlusion}, they proposed an aggregation loss and part occlusion aware region of interest pooling to mitigate the affect of occlusion by including prior structure information of human body. 
\fi






\noindent\textbf{Pedestrian detection benchmarks.}
Over the years, several datasets for pedestrian detection have been created such as Town Center \cite{benfold2011stable}, USC \cite{wu2007cluster}, Daimler-DB \cite{munder2006experimental}, INRIA \cite{dalal2005histograms}, ETH \cite{ess2007depth}, and TUDBrussels \cite{wojek2009multi}. 
All of the aforementioned datasets were typically collected for surveillance application. 
None of these datasets were created with the aim of providing large-scale images for the autonomous driving systems. 
However, in the last decade several datasets have been proposed from the context of autonomous driving such as KITTI \cite{geiger2012we}, \caltech{}, \cityperson{} and \ecp{}. Typically these datasets are captured by a vehicle-mounted camera navigating through crowded scenarios. 
These datsets have been used by several methods with \caltech{} and \cityperson{} being the most established benchmarks in this domain. 
However, \caltech{} and \cityperson{} datasets are monotonous in nature and they lack diverse scenarios (contain only street view images). 
Recently, \ecp{} dataset which is an order of magnitude larger than \cityperson{} has been porposed. 
\ecp{} is much bigger and diverse as it contains images from all seasons, under both day and night times, in several different countries. 
However, despite its large scale, \ecp{} provides a limited diversity (in terms of scene and background) and density (number of people per frame is less than 10). 
Therefore, in this paper we argue that despite some recent large scale datasets, the ability of pedestrian detectors to generalize has been constrained by lack of diversity and density. 
Moreover, benchmarks such as WiderPerson~\cite{zhang2019widerpersondataset} \widerperson{} and \crowdhuman{}, which contain web crawled images provide a much larger diversity and density. 
This enables detectors to learn a more robust representation of pedestrians with increased generalization ability. 


\noindent\textbf{Cross-dataset evaluation.}
Previously, other works \cite{braun2018eurocity,shao2018crowdhuman,zhang2017citypersons} have investigated the role of diverse and dense datasets in the performance of pedestrian detectors. 
Broadly, these works focused on the aspect that how much pre-training on a large-scale dataset helps in the performance of a pedestrian detector and used cross-dataset evaluation for this task. However, in this work we adopt cross-dataset evaluation to test the generalization abilities of several state-of-the-art pedestrian detectors.
Under this principal, we illustrate that current state-of-the-art detectors lack in generalization, whereas a general object detector generalizes performs and through a progressive training pipeline significantly surpasses current pedestrian detectors. 
Moreover, we include more recent pedestrian detection benchmarks in our evaluation setup. 

 


% With the prevalence of deep convolutional neural
% network, which has achieved impressive results in various domains, most recent
% pedestrian detection methods are CNN-based. Many methods were variations
% of Faster R-CNN [35] which has shown great accuracy in general object detection. RPN+BF [43] replaced the downstream classifier of Faster R-CNN with
% a boosted forest and used aggregated features with a hard mining strategy to
% boost the small size pedestrian detection performance. SA-FastRCNN [19] and
% MS-CNN [5] extended Fast and Faster R-CNN [15, 35] with a multi-scale network
% to deal with the scale variations problem, respectively. Instead of a single downstream classifier, F-DNN [11] employed multiple deep classifiers in parallel to
% post verify each region proposal using a soft-reject strategy. Different from these
% two stages methods, our proposed approach directly outputs detection results without post-processing [23, 34]. Apart the above full-body detectors, several
% human part based methods [12, 31, 32, 37, 47, 48] have been introduced to handle
% occlusion issues. These occlusion-specific methods learned a set of part-detector,
% where each one was responsive to detect a human part. The results from these
% part detections were then fused properly for locating partially occluded pedestrians. The occlusion-specific detectors were able to give a high confidence score
% based on the visible parts when the full-body detector was confused by the presence of background. Instead of part-level classification, we explore pixel-level
% masks which guide the detector to pay more attention to human body parts.


==> sections/sup_intro.tex <==
\section{Introduction}
\label{sec:intro}
This supplementary material provides some example images of different datasets for pedestrian detection. Additionally, quantitative and qualitative results are also shown and discussed. 

Please watch the attached {\tt supmat1.mp4} and {\tt supmat2.mp4} for more qualitative results. In particular, the videos illustrate the performance of Cascade RCNN across different locations and under varying conditions.



\section{Dataset Illustrations}

We showcase some examples of datasets related to pedestrian detection in Figure \ref{fig:dat-exp}. Top row depicts different scenarios in diverse and dense datasets collected by crawling on web. Bottom row illustrates images from traditional autonomous driving datasets. It can be observed that web-crawled datasets provide more enriched representation of pedestrians, since they cover several scenarios, such as different poses, illumination and different types of occlusion. Whereas, autonomous driving benchmarks are monotonous in nature, i.e. same background, view-point etc. Interestingly, \ecp{} and \cityperson{}, illustrate striking resemblance (where the camera is mounted, image resolution, geographical location etc.), this further stresses the point that, it is reasonable to expect that pedestrian detector's performance would not degrade drastically, when trained on one dataset and tested on the other. 

\begin{figure*}[]
	\begin{center}
	    \includegraphics[width=1\linewidth]{images/Datasets_examples_2.png}
	   % \decoRule
	\end{center}
% 	\vspace{-5pt}
	\caption{Illustration of benchmarks. Top row shows images from diverse and dense datasets, such as \crowdhuman{} and \widerperson{}. Bottom row presents images of autonomous driving benchmarks, \ecp{}, \cityperson{} \caltech{}
	}
	\label{fig:dat-exp}
\end{figure*}
 

\section{Pedestrian Detectors and Progressive Training Pipeline}
In Table \ref{tab:icon-collapsed}, we show results of CSP\cite{Liu2018DBC} (with HRNet) and Cascade RCNN\cite{cai2019cascade}. Intuitively, progressive training pipeline improved both methods. However, in the case of CSP, even with pre-training on two large-scale datasets, performance is not better than direct dataset training (when train on CityPersons, cf. Table 6, second row in the paper). Importantly, CSP and its extensions such as BGCNet \cite{li2020box}, rely on center-line annotations with a fixed aspect ratio of bounding boxes, as done in CityPersons and Caltech dataset (see Table 1 of the paper). Therefore, for CSP, exact center point is of paramount importance and whenever the annotation is not center-line, CSP would suffer a deterioration in the performance (another example of target set adaptation). In contrast, Cascade R-CNN performs better in comparison with its direct dataset performance by a significant margin. This is coherent with our previous finding, pedestrian detector like CSP, does not exploit large scale dataset like a general object detector such as Cascade RCNN does, because of generic design and no particular target set adaptation.

Finally, we add the training part of our target set to our progressive training pipeline as illustrated in Table \ref{tab:icon-collapsed2}. Although this paper stresses the importance of cross-dataset evaluation, for the sake of completeness, we also include results for target set fine-tuning. Visible improvement across all splits can be observed for both methods. Interestingly, on CityPersons, CSP gets better than Cascade RCNN. We attribute this to the fact that CSP's design choice is optimized for CityPersons (at the cost of generalization). Therefore, it benefits more than a general design object detector for target set fine-tuning on CityPersons. However, both methods are still comparable and in the case of Caltech, Cascade R-CNN outperforms CSP significantly. Moreover, the performance on Caltech is nearly in the same order, as that of humans (0.88). This also brings to the conclusion that Caltech dataset is almost solved. Next generation pedestrian detectors should use Caltech as a reference, but focus on more challenging dataset such as ECP and CityPersons. Importantly, general object detector such as, Cascade RCNN, without fine-tuning on the target set (cf. Table \ref{tab:icon-collapsed}), can already achieve comparable results to that with fine-tuning as in Table \ref{tab:icon-collapsed2}, making it practical, ready to use and more suitable to real-world problems. 


\begin{table*}[tb]
\centering
\caption{Investigating the effect on performance when CrowdHuman, Wider Pedestrian and ECP are used for progressive fine-tuning.}
\label{tab:icon-collapsed}
%  \resizebox{0.98\linewidth}{!}{
\begin{tabular}{l|c|c|c|c|c}
\hline
Method & Training        & Testing     & Reasonable & Small & Heavy \\ \hline
Casc. RCNN&CrowdHuman $\rightarrow$ ECP & CP & {10.3}     & {12.6}   & {40.7}  \\ \hline
CSP&CrowdHuman $\rightarrow$ ECP & CP & {10.4}     & {10.0}   & {36.2}  \\ \hline
Casc. RCNN&Wider Pedestrian $\rightarrow$ ECP & CP & \textbf{9.7}     & \textbf{11.8}  & {37.7}  \\ \hline
CSP&Wider Pedestrian $\rightarrow$ ECP & CP & {9.8}     & {14.6}  & \textbf{35.4}  \\ 
\hline \hline 
Casc. RCNN&CrowdHuman $\rightarrow$ ECP & Caltech & {2.9}     & {11.4}   & {30.8}  \\ \hline
CSP&CrowdHuman $\rightarrow$ ECP & Caltech & {11.0}     & {14.7}   & {32.2}  \\ \hline
Casc. RCNN &Wider Pedestrian $\rightarrow$ ECP & Caltech & \textbf{2.5}     & \textbf{9.9}   & \textbf{31.0}  \\ \hline
CSP &Wider Pedestrian $\rightarrow$ ECP & Caltech & {8.6}     & {12.0}   & {30.3}  \\ \hline
\end{tabular}
%}
\end{table*}

\begin{table*}[tb]
\centering
\caption{After fine-tuning on the target set.}
\label{tab:icon-collapsed2}
%  \resizebox{0.98\linewidth}{!}{
\begin{tabular}{l|c|c|c|c|c}
\hline
Method & Training        & Testing     & Reasonable & Small & Heavy \\ \hline
Casc. RCNN&CrowdHuman $\rightarrow$ ECP $\rightarrow$ CP & CP & {8.0}     & {8.5}   & {27.0}  \\ \hline
CSP&CrowdHuman $\rightarrow$ ECP $\rightarrow$ CP & CP & {8.1}     & {8.9}   & {29.3}  \\ \hline
Casc. RCNN&Wider Pedestrian $\rightarrow$ ECP $\rightarrow$ CP & CP & {7.5}     & {8.0}  & {28.0}  \\ \hline
CSP&Wider Pedestrian $\rightarrow$ ECP $\rightarrow$ CP & CP & \textbf{7.1}     & \textbf{7.8}  & \textbf{26.9}  \\ 
\hline \hline 
Casc. RCNN&CrowdHuman $\rightarrow$ ECP $\rightarrow$ Caltech & Caltech & {2.2}     & {8.1}   & {30.7}  \\ \hline
CSP&CrowdHuman $\rightarrow$ ECP $\rightarrow$ Caltech & Caltech & {3.8}     & {9.2}   & {31.2}  \\ \hline
Casc. RCNN &Wider Pedestrian $\rightarrow$ ECP $\rightarrow$ Caltech & Caltech & \textbf{1.7}     & \textbf{7.2}   & \textbf{25.7}  \\ \hline
CSP &Wider Pedestrian $\rightarrow$ ECP $\rightarrow$ Caltech & Caltech & {2.4}     & {7.5}   & {30.3}  \\ \hline
\end{tabular}
%}
\end{table*}




\begin{table}[tb]
\centering
\caption{Results on the withheld Test Set of CityPersons.}
\label{tab:cp-test}
 \resizebox{0.98\linewidth}{!}{
\begin{tabular}{l|c|c|c}
\hline
Methods             & Reasonable & Small & Heavy \\ \hline
MS-CNN \cite{cai2016unified}	&13.32 &	15.86 &	51.88 \\ \hline
FRCNN \cite{zhang2017citypersons}	& 12.97 &	37.24	& 50.47 \\ \hline
Cascade MS-CNN \cite{cai2019cascade}	& 11.62 &	13.64 & 47.14 \\ \hline
Repulsion Loss \cite{wang2018repulsion} &	11.48	& 5.67 &	52.59   \\ \hline
AdaptiveNMS \cite{liu2019adaptive} &  11.40     & 13.64  & 46.99   \\ \hline
OR-CNN \cite{zhang2018occlusion}  &  11.32     & 14.19 & 51.43   \\ \hline
HBA-RCNN \cite{lu2019semantic} &  11.26     & 15.68  & 43.7   \\ \hline
MGAN \cite{pang2019maskguided}  &  9.29     & 11.38  & 40.97   \\ \hline
%APD \cite{zhang2019attributeaware}  &  8.27     & 11.03  & 35.45   \\ \hline
CrowdHuman $\rightarrow$ECP$\rightarrow$CP \textsuperscript{$\ddagger$}   & 8.35     & 9.85  & 27.87   \\ \hline
WiderPerson$\rightarrow$ECP$\rightarrow$CP \textsuperscript{$\ddagger$}   & 8.31     & 10.23  & 28.18   \\ \hline
Ensemble \textsuperscript{$\ddagger$} & \textbf{7.69}     & \textbf{9.16}   & \textbf{27.08}  \\ \hline
\end{tabular}
}
\end{table}

\section{Quantitative Results on Leaderboard}

We further evaluated proposed training pipeline along with ensemble of our two models, one pre-trained on \crowdhuman{} and the other one on \widerperson{}. Ensembling is performed by combining the detections followed by non-maxima suppression, using soft-nms \cite{bodla2017soft}. 
Final results are evaluated on the dedicated server\footnote{\url{https://github.com/cvgroup-njust/CityPersons}\\
\url{https://eurocity-dataset.tudelft.nl/eval/benchmarks/detection} \\
\textsuperscript{$\ddagger$}: Correspond to our submissions and use of additional training data\\
\label{ftnote}}
(test set annotations are withheld) of \cityperson{} and \ecp{}, maintained by the benchmark publishers and frequency of submissions are constraint. Moreover, we have included results only for the published methods (detailed evaluations of all methods can be seen on the urls provided in the \emph{footnote} \ref{ftnote}). Results are presented in Table \ref{tab:cp-test} and \ref{tab:ecp-test}. Our submission (Cascade RCNN)  achieves 1st and 2nd on both leaderboards respectively. These results serve as a reference for future methods. However, no other method to the best of our knowledge uses extra training data. Therefore, giving our submissions an unfair advantage. Finally, as stated above, fine-tuning on target set is not the goal of the paper and in many cases it is not practical. In this work, we argue in the favor of cross-dataset evaluation and its importance.   










\begin{table}[t]
\centering
\caption{Results on the withheld Test Set of ECP.}
\label{tab:ecp-test}
 \resizebox{0.98\linewidth}{!}{
\begin{tabular}{l|c|c|c}
\hline
Training             & Reasonable & Small & Heavy \\ \hline
%WiderPerson + CrowdHuman + ECP & Caltech    &  1.89    &   8.1   & 26.11  \\ \hline
R-FCN (with OHEM) \cite{braun2018eurocity} &  16.3    & 24.5  & 50.7  \\ \hline
SSD \cite{braun2018eurocity} &  13.1    & 23.5  & 46.0  \\ \hline
Faster R-CNN \cite{braun2018eurocity}  & 10.1     & 19.6  & 38.1   \\ \hline
YOLOv3 \cite{braun2018eurocity} &   9.7   & 18.6  & 40.1  \\ \hline
%SPNet \cite{jiang2020sp} & 5.3     & 11.7   & \textbf{24.5} % \\ \hline
CrowdHuman$\rightarrow$ECP \textsuperscript{$\ddagger$} & 6.6     & 13.6  & 31.3  \\ \hline
%\hline
WiderPerson$\rightarrow$ECP \textsuperscript{$\ddagger$}   & {5.5}     & {11.7}   & {26.1}  \\ \hline
Ensemble \textsuperscript{$\ddagger$}  & {5.1}     & {11.2}   & 25.4  \\ \hline
SPNet \cite{jiang2020sp} & \textbf{4.2}     & \textbf{9.5}   & \textbf{21.6}  \\ \hline
\end{tabular}
}
\end{table}









\section{Qualitative Results}

We show detection quality of \ours{} on different datasets in Figure \ref{fig:good-1}. Top row contain results from \caltecha{} and bottom row show images from \citypersona{} and \ecpa{}. One could observe that \ours{} is robust to crowd density, as presented images show several instances of occlusion, people walking in close vicinity, etc. 
Furthermore, we extracted images from different regions across the globe under varying conditions, shown in Figure, \ref{fig:good-2}. Four different conditions are showcased, for example, Netherlands shows rainy conditions, where people are wearing jackets with hood, rain coats and holding umbrellas. In Italy, summer season is illustrated and people are walking in city-center in close vicinity, often occluding each other. Winter season can be seen in Germany, as snow is visible. Finally, France illustrates a low-illumination scenario, where car headlights can be seen illuminating the scene (also bringing reflections and shadows into play). Aim of this figure is to demonstrate the robustness of \ours{}, since the pre-training is done on web-crawled datasets and thanks to the several diverse and dense scenes, \ours{} has learnt a representation capable of handling several real-world scenarios efficiently. 

Finally, we show qualitatively in Figure \ref{fig:gen-com}, how pedestrian detectors such as CSP lacks in generalization compared with a general object detector such as Cascade RCNN. In the figure \ref{fig:gen-com}, we trained both detectors with HRNet on CityPersons and evaluate on ECP. We picked cases from different cities, under varying lighting conditions (afternoon, evening etc.) and under different weathers such as sunny, raining or snowing. Common failure cases for CSP includes low-illumination/blurry  pedestrians Fig.\ref{fig:gen-com} \textbf{(a)} and \textbf{(d)}, small-scale pedestrians Fig.\ref{fig:gen-com} \textbf{(g)} to \textbf{(l)}, and occlusion Fig.\ref{fig:gen-com} \textbf{(b, c, e, f, k)}. On the contrary, Cascade RCNN seems to be robust to such domain shifts and handles the above mentioned challenging scenarios better than CSP. We argue that probable reasons behind CSP's poor generalizations stems from the fact that it is a single stage detector without feature alignment compared to two-stage detector like Cascade RCNN. Feature alignment improves generalization \cite{chen2019synergistic}. Moreover, two-stage detectors have specific module for feature-alignment (ROI-Align), therefore leading them to more aligned features on unseen domains. This explicit feature alignment is absent in CSP and on unseen domains leads to failure cases, such as occlusion and small-scale pedestrians, where feature alignment becomes pivotal for precise localization. 




% We argue, that reasons behind CSP's poor generalizations stems from the fact that CityPersons is a relatively smaller dataset (around 2000 images in the training set). Another evidence of such claims exist in Table \ref{tab:icon-collapsed} and \ref{tab:icon-collapsed2}, where by adding more data to CityPersons improves the performance of CSP more than that of Cascade RCNN. Additionally, challenging scenarios, such as, snowing or rainy conditions are quite rare to non-existent in CityPersons. Therefore, representation learnt by CSP are not robust to such domain shifts.       


 \begin{figure*}[]
	\begin{center}
	    \includegraphics[width=1\linewidth]{images/Qualit_1.png}
	   % \decoRule
	\end{center}
% 	\vspace{-5pt}
	\caption{Qualitative results of Cascade R-CNN on different benchmarks. Top row includes example from Caltech, bottom left CityPersons and ECP on bottom right. \textsuperscript{$\dagger$} }
	\label{fig:good-1}
\end{figure*}


 \begin{figure*}[]
	\begin{center}
	    \includegraphics[width=1\linewidth]{images/Qualit_2.png}
	   % \decoRule
	\end{center}
% 	\vspace{-5pt}
	\caption{Cascade R-CNN \textsuperscript{$\dagger$} across different scenarios, such as summer, winter, rain and low-illumination, illustrating the robustness of the general object detector. }
	\label{fig:good-2}
\end{figure*}



\begin{figure*}[tbh]
\begin{subfigure}{0.33\textwidth}
  \centering
  % include first image
  \includegraphics[height=0.15\textheight]{csp_sl/11_crop.jpg}
  \caption{}
  \label{fig:failures:fp:post1}
\end{subfigure}
\begin{subfigure}{0.33\textwidth}
  \centering
  % include first image
  \includegraphics[height=0.15\textheight]{csp_sl/22_crop.jpg}
  \caption{}
  \label{fig:failures:fp:post2}
\end{subfigure}
\begin{subfigure}{0.33\textwidth}
  \centering
  % include first image
  \includegraphics[height=0.15\textheight]{csp_sl/33_crop.jpg}
  \caption{}
  \label{fig:failures:fp:post3}
\end{subfigure}

\begin{subfigure}{0.33\textwidth}
  \centering
  % include first image
  \includegraphics[height=0.15\textheight]{cas_sl/11_crop.jpg}
  \caption{}
  \label{fig:failures:fp:post4}
\end{subfigure}
\begin{subfigure}{0.33\textwidth}
  \centering
  % include first image
  \includegraphics[height=0.15\textheight]{cas_sl/22_crop.jpg}
  \caption{}
  \label{fig:failures:fp:post5}
\end{subfigure}
\begin{subfigure}{0.33\textwidth}
  \centering
  % include first image
  \includegraphics[height=0.15\textheight]{cas_sl/33_crop.jpg}
  \caption{}
  \label{fig:failures:fp:post6}
\end{subfigure}

\begin{subfigure}{0.33\textwidth}
  \centering
  % include first image
  \includegraphics[height=0.15\textheight]{csp_sl/44_crop.jpg}
  \caption{}
  \label{fig:failures:fp:post7}
\end{subfigure}
\begin{subfigure}{0.33\textwidth}
  \centering
  % include first image
  \includegraphics[height=0.15\textheight]{csp_sl/55_crop.jpg}
  \caption{}
  \label{fig:failures:fp:post8}
\end{subfigure}
\begin{subfigure}{0.33\textwidth}
  \centering
  % include first image
  \includegraphics[height=0.15\textheight]{csp_sl/66_crop.jpg}
  \caption{}
  \label{fig:failures:fp:post9}
\end{subfigure}

\begin{subfigure}{0.33\textwidth}
  \centering
  % include first image
  \includegraphics[height=0.15\textheight]{cas_sl/44_crop.jpg}
  \caption{}
  \label{fig:failures:fp:post10}
\end{subfigure}
\begin{subfigure}{0.33\textwidth}
  \centering
  % include first image
  \includegraphics[height=0.15\textheight]{cas_sl/55_crop.jpg}
  \caption{}
  \label{fig:failures:fp:post12}
\end{subfigure}
\begin{subfigure}{0.33\textwidth}
  \centering
  % include first image
  \includegraphics[height=0.15\textheight]{cas_sl/66_crop.jpg}
  \caption{}
  \label{fig:failures:fp:post13}
\end{subfigure}


	\caption{Generalization comparison between CSP \cite{Liu2018DBC} with HRNet and Cascade RCNN\cite{cai2019cascade}. Both methods are trained on CityPersons and evaluated on ECP. Images with Yellow bounding box are CSP's detections where as magenta bounding box are Cascade RCNN's detections. Dotted green line illustrates instances where CSP fails to detect.}
	\label{fig:gen-com}
\end{figure*}


\section{Errata}
We will fix the typographical error occurring in the manuscript such as, on lines 718, 647, 683 and 761.
% Line 718-719 Table 8, caption, there is an redundant and in the caption.
% Line 647, uppercase I
% Line 683 from is missing 761, typographical error dataset


% \subsection{Discussion: Failure Cases}
% \ours{}, like other state-of-the-art pedestrian detectors, performs quite well for non-occluded, large pedestrians in upright pose but its performance decreases significantly (approximately by a factor of 4) for heavily occluded pedestrians and by few percentage points for small (i.e. far away from camera) pedestrians.
% %  widely known \cite{braun2018eurocity} that their
% This drop in performance is intuitive as these are often challenging cases where even human annotators may sometime dis-agree or require careful examination to detect and localize pedestrians.


% When deploying a pedestrian detector in a real-world applications, it is important to know the scenarios where it could fails. 
% So, in this section, we focus on the false positive (FP) and false negative (FN) errors of \ours{} which are relatively easy for a human annotator.

% \begin{figure}[tbh]
% \begin{subfigure}{0.1\textwidth}
%   \centering
%   % include first image
%   \includegraphics[height=0.17\textheight]{images/fp-posters/FP_0.985072672367096_brno_01090_10.jpg}
%   \caption{}
%   \label{fig:failures:fp:post1}
% \end{subfigure}
% \bigskip % force a bit of vertical whitespace
% \begin{subfigure}{0.09\textwidth}
%   \centering
%   \includegraphics[height=0.17\textheight]{images/fp-posters/FP_0.9115092754364014_ulm_00675_10.jpg}
%   \caption{}
%   \label{fig:failures:fp:post2}
% \end{subfigure}
% % \begin{subfigure}{0.2\textwidth}
% %   \centering
% %   % include first image
% %   \includegraphics[height=0.17\textheight]{images/fp-posters/FP_0.866519570350647_dresden_00819_10.jpg}
% %   \caption{}
% %   \label{fig:failures:fp:post3}
% % \end{subfigure}
% % \begin{subfigure}{0.2\textwidth}
% %   \centering
% %   % include first image
% %   \includegraphics[height=0.17\textheight]{images/fp-posters/FP_0.8590108156204224_brno_01075_10.jpg}
% %   \caption{}
% %   \label{fig:failures:fp:post4}
% % \end{subfigure}
% \begin{subfigure}{0.09\textwidth}
%   \centering
%   % include first image
%   \includegraphics[height=0.17\textheight]{images/fp-posters/FP_0.8063965439796448_hamburg_00706_10.jpg}
%   \caption{}
%   \label{fig:failures:fp:post5}
% \end{subfigure}
% %\vspace{-0.5}
% \begin{subfigure}{0.1\textwidth}
%   \centering
%   % include first image
%   \includegraphics[height=0.17\textheight]{images/fp-signs/FP_0.9617151021957397_roma_01153_10.jpg}
%   \caption{}
%   \label{fig:failures:fp:sign1}
% \end{subfigure}
% \bigskip % force a bit of vertical whitespace
% \begin{subfigure}{0.1\textwidth}
%   \centering
%   \includegraphics[height=0.17\textheight]{images/fp-signs/FP_0.9517867565155029_roma_01173_10.jpg}
%   \caption{}
%   \label{fig:failures:fp:sign2}
% \end{subfigure}
% \begin{subfigure}{0.1\textwidth}
%   \centering
%   % include first image
%   \includegraphics[height=0.17\textheight]{images/fp-signs/FP_0.9424009919166565_potsdam_00622_10.jpg}
%   \caption{}
%   \label{fig:failures:fp:sign3}
% \end{subfigure}
% \begin{subfigure}{0.1\textwidth}
%   \centering
%   % include first image
%   \includegraphics[height=0.17\textheight]{images/fp-signs/FP_0.9089773893356323_roma_01255_10.jpg}
%   \caption{}
%   \label{fig:failures:fp:sign4}
% \end{subfigure}
% \begin{subfigure}{.1\textwidth}
%   \centering
%   % include first image
%   \includegraphics[height=0.17\textheight]{images/fp-signs/FP_0.8644793629646301_marseille_01502_10.jpg}
%   \caption{}
%   \label{fig:failures:fp:sign5}
% \end{subfigure}
% %\vspace{-0.5}



% \vspace{-2em}

% \begin{subfigure}{0.14\textwidth}
%   \centering
%   % include first image
%   \includegraphics[height=0.17\textheight]{images/fn-cars/FN_barcelona_01310_1_0.jpg}
%   \caption{}
%   \label{fig:failures:fn:car1}
% \end{subfigure}
% \bigskip % force a bit of vertical whitespace
% \begin{subfigure}{0.12\textwidth}
%   \centering
%   \includegraphics[height=0.17\textheight]{images/fn-cars/FN_set10_V010_I00989_1_0.jpg}
%   \caption{}
%   \label{fig:failures:fn:car2}
% \end{subfigure}
% \begin{subfigure}{0.14\textwidth}
%   \centering
%   % include first image
%   \includegraphics[height=0.17\textheight]{images/fn-cars/FN_torino_01072_1_0.jpg}
%   \caption{}
%   \label{fig:failures:fn:car3}
% \end{subfigure}
% \begin{subfigure}{0.14\textwidth}
%   \centering
%   % include first image
%   \includegraphics[height=0.17\textheight]{images/fn-cars/FN_torino_01141_1_0.jpg}
%   \caption{}
%   \label{fig:failures:fn:car4}
% \end{subfigure}
% \vspace{-1em}

% \begin{subfigure}{0.13\textwidth}
%   \centering
%   % include first image
%   \includegraphics[height=0.15\textheight]{images/fn-pose/FN_basel_00658_1_0.jpg}
%   \caption{}
%   \label{fig:failures:fn-pose1}
% \end{subfigure}
% \bigskip % force a bit of vertical whitespace
% \begin{subfigure}{0.21\textwidth}
%   \centering
%   \includegraphics[height=0.15\textheight]{images/fn-pose/FN_basel_00692_1_0.jpg}
%   \caption{}
%   \label{fig:failures:fn-pose2}
% \end{subfigure}
% \begin{subfigure}{0.24\textwidth}
%   \centering
%   % include first image
%   \includegraphics[height=0.15\textheight]{images/fn-pose/FN_bologna_01389_1_0.jpg}
%   \caption{}
%   \label{fig:failures:fn-pose3}
% \end{subfigure}
% \begin{subfigure}{0.23\textwidth}
%   \centering
%   % include first image
%   \includegraphics[height=0.15\textheight]{images/fn-pose/FN_prague_01393_1_0.jpg}
%   \caption{}
%   \label{fig:failures:fn-pose4}
% \end{subfigure}
% \begin{subfigure}{0.1\textwidth}
%   \centering
%   % include first image
%   \includegraphics[height=0.15\textheight]{images/fn-pose/FN_set09_V004_I00839_1_0.jpg}
%   \caption{}
%   \label{fig:failures:fn-pose5}
% \end{subfigure}


% \caption{False positives (blue) and false negatives (red) for \ours{} on autonomous driving datasets at 0.1 false positive per image threshold.}
% \label{fig:failures}
% \end{figure}









% \begin{figure}[tbh]

% \begin{subfigure}{0.23\textwidth}
%   \centering
%   % include first image
%   \includegraphics[height=0.17\textheight]{images/anno-errors/FP_0.9997175335884094_toulouse_00711_10.jpg}
%   \caption{}
%   \label{fig:failures:ano-err1}
% \end{subfigure}
% \bigskip % force a bit of vertical whitespace
% \begin{subfigure}{0.23\textwidth}
%   \centering
%   \includegraphics[height=0.17\textheight]{images/anno-errors/FP_0.9999133348464966_marseille_01446_10.jpg}
%   \caption{}
%   \label{fig:failures:ano-err2}
% \end{subfigure}
% \begin{subfigure}{0.23\textwidth}
%   \centering
%   % include first image
%   \includegraphics[height=0.17\textheight]{images/anno-errors/FP_0.9999556541442871_marseille_01547_10.jpg}
%   \caption{}
%   \label{fig:failures:ano-err3}
% \end{subfigure}
% \begin{subfigure}{0.23\textwidth}
%   \centering
%   % include first image
%   \includegraphics[height=0.17\textheight]{images/anno-errors/FP_0.8687745332717896_marseille_01453_13.jpg}
%   \caption{}
%   \label{fig:failures:ano-err4}
% \end{subfigure}
% %\vspace{-0.5}

% \caption{False positives due to annotation errors.}
% \label{fig:failures2}
% \end{figure}



% Fig.~\ref{fig:failures} and ~\ref{fig:failures2} show some easy errors of \ours{}.
% False positives (FP) are shown with blue bounding boxes and false negatives (FN) are shown with red bounding boxes.
% Many of these errors (e.g. FP detections for human depictions on objects, construction workers, people entering/exiting the cars) can be attributed to lack of sufficient samples covering these types of cases in the training set.

% The FNs shown in Fig.~\ref{fig:failures:fn-pose1}-~\ref{fig:failures:fn-pose5} give a strong indication that the current model bases its prediction quite strongly on the clothes and pose of the pedestrian. If and when people are wearing unusual clothes (e.g. construction workers) or are in a relatively uncommon pose (e.g. getting in/out of a car), it struggles to detect them. 
% Therefore, it is possible that the current detector despite achieving good results on popular pedestrian detection benchmarks might degrade in places and scenarios where the pedestrian are involved in different activities and/or are wearing different clothing.
% Future datasets need to capture/curate images from a much wider range of countries and scenarios in order to ensure that a more complete range of poses and appearances are captured.

% Another interesting set of FP failures, Fig~\ref{fig:failures:fp:sign1}-\ref{fig:failures:fp:sign5}, is due to traffic signs/lights whose poles are occluded by cars.
% In several such instances, the shape of the sign (round) resembles an occluded pedestrian's head but the appearance is quite different, yet the model makes a false detection.
% This indicates that the model is giving more weight to the shape in these cases and much lower weight to the appearance.
% %Though, it is reasonable that appearance of non-occluded head, in these cases, can vary a lot, whereas the shape is much more constrained.
% Using hard-negative mining for these cases can potentially resolve these errors and may reduce similar FPs.

% \ours{} also sometimes fails to detect people entering/exiting a car, Fig.~\ref{fig:failures:fn:car1}-\ref{fig:failures:fn:car4}.
% In some of these cases, the person is partially occluded which makes the detection challenging. 
% Nevertheless, the size of pedestrian and the visible part is large enough for a human to easily detect them.
% The likely reason for the failure of \ours{} to detect them is the unusual pose that these pedestrians have compared to typical pedestrian poses. 
% Since, current autonomous datasets consist of images from a car, these types of poses are not frequent.
% This indicates that to develop more robust pedestrian detectors, which can handle this type of relatively rare poses, rare cases have to be actively curated/captured.

% A substantial proportion of \ours{}'s false positive (FP) detections at 0.1 FP/image threshold are actually due to annotation errors.
% Fig.~\ref{fig:failures2} shows some of the easier FP errors due to these annotation errors.
% %pedestrians 
% %In case of heavily occluded pedestrians, these annotation errors are more common.

% %The children are over-represented in the FNs. 
% %This could be partly due to the fact that children are under-represented in the training set or due to the smaller size of children.

% %Another interesting set of failures is due to the presence of animals, e.g. dogs and horses.


% %There are also many FNs in the vicinity of bicycles.
% %This is probably due to inconsistency in the annotation of ignore regions as .

% \clearpage
